Blindfolded Attackers Still Threatening: Strict Black-Box Adversarial Attacks on Graphs

Adversarial attacks on graphs have attracted considerable research interests. Existing works assume the attacker is either (partly) aware of the victim model, or able to send queries to it. These assumptions are, however, unrealistic. To bridge the gap between theoretical graph attacks and real-world scenarios, in this work, we propose a novel and more realistic setting: strict black-box graph attack, in which the attacker has no knowledge about the victim model at all and is not allowed to send any queries. To design such an attack strategy, we first propose a generic graph filter to unify different families of graph-based models. The strength of attacks can then be quantified by the change in the graph filter before and after attack. By maximizing this change, we are able to find an effective attack strategy, regardless of the underlying model. To solve this optimization problem, we also propose a relaxation technique and approximation theories to reduce the difficulty as well as the computational expense. Experiments demonstrate that, even with no exposure to the model, the Macro-F1 drops 6.4% in node classification and 29.5% in graph classification, which is a significant result compared with existent works.

==> impact.tex <==
%!TEX root = eigentack.tex

\section{Ethics Statement}
\label{sec:impact}
Recently, deep learning on graphs has shown excellent results in different real-world applications including molecule analysis~\cite{hamilton2017inductive}, drug discovery~\cite{gilmer2017neural}, financial surveillance~\cite{paranjape2017motifs}, recommendation systems~\cite{wang2019knowledgeaware}, \emph{etc.} These breakthroughs are attributed to advances in the development of graph learning models (\emph{e.g.} graph neural networks, node/graph representation methods), as well the availability of dealing with huge amounts of graph data and computational power. Despite these impressive results, the research community has recently shown that graph learning models are vulnerable to adversarial attacks~\cite{chen2020survey, bojchevski2019adversarial, dai2018adversarial, zugner2019adversarial}.

A graph attacker can intentionally modify the original graph such that the modifications are almost human-imperceptible, which can cause wrong predictions in graph learning models. The real-life applications of such attacks can be very serious, for instance, one could create some false connections with rich people to increase his/her credit score in an online payment company, then he/she will be able to get loan and run away from the system. 
For that reason, we are interested in understanding these attacks to discover various inherent threats in practical applications such that we can better prevent or block the malwares and hackers.

In this paper, we introduce a query-free black-box adversarial attack on graphs, where the attacker has no knowledge of the target model and no query access to the model. If the attack model is maliciously utilized by someone while the target lacks awareness of prevention, this could increase the risk of the model or its outputs being misclassified. 
Nevertheless, the attack model also provides us a novel way to better understand the vulnerability of graph learning models, thus motivate us to provide better defense way or more robust models when facing with such graph adversarial attacks.
For example, the most straightforward defense way is to inject adversarial examples to adversarial learning such that the trained model can correctly classify the future adversarial examples. 
Accordingly, whether the technology can bring negative or beneficial impacts to the society depends on whether the bad-motivated or well-motivated users can take advantage of this technology, and we suggest that people should be cautious of such graph adversarial attacks when designing their graph learning models.
We would also encourage further works to develop better defense methods against such attacks. 

% This work may have some negative consequences because the adversarial attack model on graphs is likely to be used maliciously to spread misinformation and some people can profit from it. Nevertheless, it also provides a novel way to inject adversarial examples to adversarial learning when defending graph learning models such that the trained model can correctly classify the future adversarial examples.
